Regularizing Black-box Models for Improved Interpretability

Most of the work on interpretable machine learning has focused on designing either inherently interpretable models, which typically trade-off accuracy for interpretability, or post-hoc explanation systems, whose explanation quality can be unpredictable. Our method, ExpO, is a hybridization of these approaches that regularizes a model for explanation quality at training time. Importantly, these regularizers are differentiable, model agnostic, and require no domain knowledge to define. We demonstrate that post-hoc explanations for ExpO-regularized models have better explanation quality, as measured by the common fidelity and stability metrics. We verify that improving these metrics leads to significantly more useful explanations with a user study on a realistic task.

==> sections/scratch.tex <==
\begin{figure}[t]
    \centering
    \floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,center},capbesidewidth=0.4\textwidth}}]{figure}[\FBwidth]
    {\caption{%
    The effects of our regularizer on a model predicting Bob's credit rating.
    The abrupt kinks in the unregularized model make the local linear approximations both less faithful to the model and less stable to small perturbations.  
    The regularized model is much smoother and therefore easier to explain.  
    Also observe that, when over-regularized, we can force the learned function to be essentially linear.}%
    \label{fig:toy}}
    {\includegraphics[width=0.5\textwidth]{figures/ToyExample.png}}
\end{figure}
